Multi-lingual Common Semantic Space Construction via Cluster-consistent Word Embedding

We construct a multilingual common semantic space based on distributional semantics, where words from multiple languages are projected into a shared space to enable knowledge and resource transfer across languages. Beyond word alignment, we introduce multiple cluster-level alignments and enforce the word clusters to be consistently distributed across multiple languages. We exploit three signals for clustering: (1) neighbor words in the monolingual word embedding space; (2) character-level information; and (3) linguistic properties (e.g., apposition, locative suffix) derived from linguistic structure knowledge bases available for thousands of languages. We introduce a new cluster-consistent correlational neural network to construct the common semantic space by aligning words as well as clusters. Intrinsic evaluation on monolingual and multilingual QVEC tasks shows our approach achieves significantly higher correlation with linguistic features than state-of-the-art multi-lingual embedding learning methods do. Using low-resource language name tagging as a case study for extrinsic evaluation, our approach achieves up to 24.5\% absolute F-score gain over the state of the art.

==> 5analysis.tex <==
\section{Analysis}

%\lifu{Impact of number of bilingual lexicons}
In order to show the impact of the size of bilingual lexicons, we reduce the size of the original lexicons for these three languages from 400,00 to 100,00 and to 50,00. For fair comparison, we use MultiCCA as the major baseline. Table~\ref{3lang5000} shows the results. We can see that, the MultiCCA approach is very sensitive to the size of the bilingual lexicon, while our approach can perform much better when the bilingual lexicon size is 100,00 or 20,00. 

\begin{table*}[!htp]
\small
%\scriptsize
\footnotesize
\begin{center}
\begin{tabular}{p{1.0cm}|p{1.9cm}|p{2.35cm}<{\centering}|p{2.35cm}<{\centering}|p{2.55cm}<{\centering}|p{2.35cm}<{\centering}}
\hline
\multicolumn{2}{p{2.6cm}<{\centering}|}{} &  Monolingual QVEC & Multilingual Qvec & Monolingual Qvec-CCA & Multilingual Qvec-CCA\\
 \hline
 \multirow{2}{1.0cm}{40,000} & multiCCA  & 10.7 & 8.8 & 63.5 & 41.5 \\
 %\cline{2-9}
& CorrNets & 14.7 & 11.1 &  63.2 & 41.3 \\
% & Our Approach & 40.1 & 50.5 & 47.4 & 15.5 & \textbf{12.7} & \textbf{66.5} & \textbf{46.3} 
& Our Approach  & \textbf{15.4} & \textbf{12.6} & \textbf{66.4} & \textbf{44.4} \\
\hline
%\hline
\multirow{2}{1.0cm}{10,000} & multiCCA  & 9.7 & 6.1 & 63.2 & 40.1 \\
 %\cline{2-9}
& CorrNets  & 14.8 & 11.2 & 63.1 & 41.0 \\
& Our Approach  & \textbf{15.4}  & \textbf{11.8}  & \textbf{66.0}  & \textbf{44.2} \\
% & Our Approach  & 37.9 (40.0) & 49.7 (50.9) & 35.4 (44.9) & 15.4 (15.4) & 11.8 (12.1) & 66.0 (66.4) & 44.2 (46.2) \\
%\hline
\hline
\multirow{2}{1.0cm}{2,000} & multiCCA  & 9.9 & 5.9 & 63.2 & 38.7 \\
  %\cline{2-9}
& CorrNets  & \textbf{16.3} & \textbf{13.8} & 63.1 & 39.9 \\
& Our Approach & 14.7  & 11.7  & \textbf{66.2} & \textbf{43.5} \\
% & Our Approach  & 38.8 (41.4) & 47.8 (48.9) & 27.9 (35.3) & 14.7 (14.8) & 11.7 (11.7) & 66.2 (66.6) & 43.5 (45.5) \\
 \hline
\end{tabular}
\end{center}
\caption{Comparison of the Results with Various Sizes (40,000, 10,000, 2,000) of Bilingual Lexicon}
\label{3lang5000}
\end{table*}

% \begin{table*}[!htp]
% \scriptsize
% \begin{center}
% \begin{tabular}{p{0.5cm}|p{1.4cm}|p{1.61cm}<{\centering}|p{1.61cm}<{\centering}|p{1.35cm}<{\centering}|p{1.35cm}<{\centering}|p{1.35cm}<{\centering}|p{1.35cm}<{\centering}|p{1.35cm}<{\centering}}
% \hline
% \multicolumn{2}{p{2.6cm}<{\centering}|}{} & monolingual word similarity & multilingual word similarity & Word Translation & monolingual Qvec & multilingual Qvec & monolingual Qvec-CCA & multilingual Qvec-CCA\\
%  \hline
%  \multirow{2}{1.0cm}{400,00} & multiCCA  & \textbf{43.1} & \textbf{56.4} & 33.2 & 10.7 & 8.8 & 63.5 & 41.5 \\
%  %\cline{2-9}
% & CorrNets & 39.1 & 49.0 & \textbf{40.0} & 14.7 & 11.1 &  63.2 & 41.3 \\
% % & Our Approach & 40.1 & 50.5 & 47.4 & 15.5 & \textbf{12.7} & \textbf{66.5} & \textbf{46.3} 
% & Our Approach & 37.8 & 49.2 & 38.5 & \textbf{15.4} & \textbf{12.6} & \textbf{66.4} & \textbf{44.4} \\
% \hline
% \hline
% \multirow{2}{1.0cm}{100,00} & multiCCA  & \textbf{39.7} & 45.8 & 27.7 & 9.7 & 6.1 & 63.2 & 40.1 \\
%  %\cline{2-9}
% & CorrNets  & 39.3  & 47.8  &  34.1 & 14.8 & 11.2 & 63.1 & 41.0 \\
% & Our Approach  & 37.9  & \textbf{49.7}  & \textbf{35.4}  & \textbf{15.4}  & \textbf{11.8}  & \textbf{66.0}  & \textbf{44.2} \\
% % & Our Approach  & 37.9 (40.0) & 49.7 (50.9) & 35.4 (44.9) & 15.4 (15.4) & 11.8 (12.1) & 66.0 (66.4) & 44.2 (46.2) \\
% \hline
% \hline
% \multirow{2}{1.0cm}{20,00} & multiCCA  & 38.7 & 39.1 & 7.7 & 9.9 & 5.9 & 63.2 & 38.7 \\
%   %\cline{2-9}
% & CorrNets  &  35.7 & 43.2 & 16.6 & \textbf{16.3} & \textbf{13.8} & 63.1 & 39.9 \\
% & Our Approach  & \textbf{38.8} & \textbf{47.8} & \textbf{27.9} & 14.7  & 11.7  & \textbf{66.2} & \textbf{43.5} \\
% % & Our Approach  & 38.8 (41.4) & 47.8 (48.9) & 27.9 (35.3) & 14.7 (14.8) & 11.7 (11.7) & 66.2 (66.6) & 43.5 (45.5) \\
%  \hline
% \end{tabular}
% \end{center}
% \caption{Comparison of the Results with Various Sizes (400,00, 100,00, 20,00) of Bilingual Lexicon}
% \label{3lang5000}
% \end{table*}
 
%\lifu{Impact of number of languages}


